How Functional Complexity affects the Scalability-Energy Efficiency Trade-Off of HCC WSN Clustering

Even though clustering algorithms in Wireless Sensor Networks (WSN) are a well investigate subject, the increasing interest in the Internet of Things (IoT) and 5G technologies has precipitated the need of new ways to comprehend and overcome a new set of challenges. While studies mainly propose new algorithms and compare these algorithms based on a set of properties (e.g. energy efficiency, scalability), none of them focuses on the underlying mechanisms and organizational patterns that lead to these properties. We address this lack of understanding by applying a complex systems science approach to investigate the properties of WSNs arising from the communication patterns of the network nodes. We represent different implementations of clustering in WSNs with a functional topology graph. Moreover, we employ a complexity metric - functional complexity (CF) - to explain how local interactions give rise to the global behavior of the network. Our analysis shows that higher values of CF indicate higher scalability and lower energy efficiency.

==> Clustering in WSNs Abstract/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Communications Society subset of the full
IEEEtran package and is intended for use with IEEE Communications Society
publications. The included version of the IEEEtran_HOWTO.pdf has been
specially formatted in IEEE Communications Society (comsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf,
                   bare_jrnl_comsoc.tex.
***************************************************************************


==> Clustering in WSNs Abstract/abstract_section.tex <==
% !TeX spellcheck = en_US
\textcolor{activecolor}{Even though clustering algorithms in Wireless Sensor Networks (WSN) are a well investigate subject, the increasing interest in the Internet of Things (IoT) and 5G technologies has precipitated the need of new ways to comprehend and overcome a new set of challenges. While studies mainly propose new algorithms and compare these algorithms based on a set of properties (e.g. energy efficiency, scalability), none of them focuses on the underlying mechanisms and organizational patterns that lead to these properties. We address this lack of understanding by applying a complex systems science approach to investigate the properties of WSNs arising from the communication patterns of the network nodes.} We represent different implementations of clustering in WSNs with a functional topology graph. Moreover, we employ a complexity metric - functional complexity ($C_F$) - to explain how local interactions give rise to the global behavior of the network. Our analysis shows that higher values of $C_F$ indicate higher scalability and lower energy efficiency.  

%predlazu rjesenja koja predstavljaju nove algoritme i porede svoja rjesenja sa drugim algoritmima, mi predlazemo framework koji bi nam omogucio da razumijemo strukturne karakteristike koje underpin te algoritme. 
%ISKORISTITI OVU KONSTRUKCIJU DA KAZEMO DA NIKO NIJE OBJASNIO RAZLOG STVARI KOJE UNDERPIN SVA RJESENJA I KOJA DOVODE DO ODGOVARAJUCIH KARAKTERISTIKA ---- While several studies have been made to quantify the number of spectrum opportunities potentially obtained through the use of such mechanism, none of them focuses on how it would be implemented on a real-time radio system.




%In order to understand the underlying mechanisms that lead to certain network properties (i.e. scalability, energy efficiency) we apply a complex systems science approach to analyze clustering in Wireless Sensor Networks (WSN). We represent different implementations of clustering in WSNs with a functional topology graph. Different characteristics of the functional topology provide insight into the relationships between system parts that result in certain properties of the whole system. Moreover, we employ a complexity metric - functional complexity ($C_F$) - to explain how local interactions give rise to the global behavior of the network. Our analysis shows that higher values of $C_F$ indicate higher scalability and lower energy efficiency.  

%\hl{Our analysis shows that a longer average path length of the functional topology results in lower energy efficiency of the modeled clustering implementation.} 


%The constant desire to automate processes that intertwine different aspects of human life results in the need to connect everything that surrounds us. The evolution of electronic devices that can sense the environment, talk to each other, and process the sensing information allows us to build networks of sensors. Such networks, if designed properly, prove themselves useful in many applications, including smart cities, environmental monitoring, and military field surveillance. 
%The idea of a connected world dates back to the very beginning of network development. 

==> Clustering in WSNs Abstract/acknowledgment_section.tex <==
% !TeX spellcheck = en_GB
This material is based upon works supported by the Science Foundation Ireland under the Grant No. 13/RC/2077.

==> Clustering in WSNs Abstract/acronyms_section.tex <==
% !TeX spellcheck = en_GB
\begin{acronym}
	\acro{RNC}{Radio Network Controler}
	\acro{nodeB}{UMTS base transciever station}
	\acro{VLR}{Visitor Location Register} 
	\acro{HLR}{Home Location Register}
	\acro{SGSN}{Serving GPRS Support Node}
	\acro{MSC}{Mobile Switching Center}
	\acro{SMS}{Short Message Service}
	\acro{IoT}{Internet of Things}
	\acro{AP}{Access Points}
	\acro{WSNs}{Wireless Sensor Networks}
	\acro{WSN}{Wireless Sensor Network}
	\acro{IoT-GSI}{Global Standards Initiative on Internet of Things}
	\acro{DCA}{Distributed Clustering Algorithm}
	\acro{BFS}{Breadth-First Search}
	\acro{LEACH}{Low Energy Adaptive Clustering Hierarchy}
	\acro{HCC}{Hierarchical Control Clustering}
	\acro{HEED}{Hybrid Energy-Efficient Distributed}
\end{acronym}


==> Clustering in WSNs Abstract/analysis_section.tex <==
% !TeX spellcheck = en_US
\textcolor{activecolor}{Adding a new node to a cluster created according to the \ac{HCC} algorithm simply means that the new node gets connected to one of the existing nodes which is going to be its parent node. The new node does not need to inform all nodes in the cluster about its arrival, which simplifies the process of adding nodes to the network and represents a highly scalable implementation. According to the authors of \cite{Abbasi2007,Liu2012, Aslam2012} and \cite{Jiang2009} hierarchical approaches proved themselves to be more scalable than their non-hierarchical counterpart. The authors of \cite{Jiang2009} showed that a trade-off exists between network scalability and energy consumption in clustering schemes. Our goal is to investigate the relationship between these objectives and the functional complexity, which would allow us to analyze them together.}

\begin{figure}[t]
	\centering
	\includegraphics[scale=0.4]{pics/complexity_hcc_4x5}      
	\caption{Functional complexity of the \ac{HCC} algorithm; the functional complexity is the area between the green and the blue curves.}
	\label{complexity_hcc_4x5}
\end{figure}

\textcolor{activecolor}{Figure \ref{complexity_hcc_4x5} depicts the relationship between the uncertainty of interactions for all subset sizes and the amount of information which is expected from the calculation performed on the whole system for the \ac{HCC} algorithm, i.e. the functional complexity of \ac{HCC}. As shown in Figure \ref{functional_topology_HCCA} the functional topology of the \ac{HCC} algorithm has sparse intra and inter cluster connections. As the links in the functional topology represent functional dependencies between nodes, a sparse connectivity pattern indicates weak dependencies which result in high scalability. This follows from the fact that in order to add a node to the network, the new node \textcolor{second}{only needs} to establish a connection (send a message) to one of the nodes in the topology and to declare this node as its parent. The functional complexity of the \ac{HCC} algorithm is 38.31. As the authors of \cite{Abbasi2007,Liu2012, Aslam2012} and \cite{Jiang2009} agree that the communication between the cluster-head and the base station consumes most energy, an approximation of the energy efficiency could be calculated as the ratio between the average number of intra-cluster connections and the \textcolor{second}{total number} of links between the base station and each cluster-head in the functional topology.The energy efficiency of the \ac{HCC} algorithm is 0.61 which is very low.}


==> Clustering in WSNs Abstract/clustering_algorithms_section.tex <==
% !TeX spellcheck = en_US
%The importance of collecting, analyzing and interpreting data in the \ac{IoT} environment emphasizes the role of \ac{WSNs}. A WSN is a collection of connected devices (sensors), which can sense the environment, interpret the measurements and communicate this information through the network. In order to make the measurements as precise as possible, and the network as reliable as possible, \ac{WSNs} generally possess a large number of sensors. Therefore, in addition to the sensing and communication abilities, sensors have to be cheap. In order to make these devices as cheap as possible, their capabilities are limited (e.g. sensors have limited energy resources, which explicitly influences every aspect of \ac{WSNs}). 

Considering the limited energy resources and the size of \ac{WSNs}, the best approach is to partition the network into interconnected subgroups (clusters), whose local behavior gives rise to the global objective of the network (e.g. minimizing the energy consumption). Generally, clustering includes two phases:
\begin{itemize}
	\item Set-Up Phase - this phase implies choosing cluster-heads. Cluster-heads are nodes that are responsible for the coordination of the clustering process.
	\item Maintenance Phase - this phase implies reorganization of the clusters in order to add new nodes to the cluster, deal with nodes that leave the cluster, or simply change the roles of nodes (cluster-head or ordinary node) in the cluster in order to achieve higher energy efficiency \cite{Basagni1999}. 
\end{itemize}

%We propose a complex systems science approach to understand how different clustering approaches lead to specific network properties (in particular we focus on scalability and energy efficiency). 
As the maintenance phase implies the reorganization of clusters in order to achieve higher energy efficiency and to adjust to changes in the topology, we focus on this phase. As mentioned previously, we consider two clustering algorithms (the \ac{LEACH} and the \ac{HCC} algorithms) proposed in \cite{Heinzelman2002} and \cite{Banerjee2001}.

\begin{figure}[t]
	\centering
	\includegraphics[scale=0.4]{pics/leach_clustering}      
	\caption{The topology created according to the \ac{LEACH} algorithm. Ordinary nodes transfer sensing information to the cluster-heads, which forward this information to the base station (The Figure is redrawn from \cite{Aslam2012})}
	\label{leach_clustering_graph}
\end{figure}

The \ac{LEACH} algorithm is based on rounds. Each round includes both phases (set-up and maintenance phase). Each node in the network runs the algorithm, and decides randomly which role to play (cluster-head or ordinary node). When a node decides to be a cluster-head it broadcasts this information, whereas each node that decided to be an ordinary node listens to the broadcast messages and joins the closest cluster-head. After all ordinary nodes join one of the cluster-heads, the set-up phase finishes and the maintenance phase starts. In the maintenance phase nodes that belong to the same cluster transfer sensing information to the cluster-head (Figure \ref{leach_clustering_graph}), and as the \ac{LEACH} algorithm involves rotating the role of cluster-heads between nodes in a cluster, the nodes that belong to the same cluster communicate to each other in order to choose the next cluster-head candidate. 
%The \ac{DCA} generalizes algorithms presented in \cite{Lin1997} and \cite{Baker1981}, by choosing the cluster-heads based on a generic weight associated with each node. Each node executes the algorithm, and each node has the knowledge of its unique identifier, its weight, and the weights and unique identifiers of its neighboring nodes. In other words, the algorithm relies only on local information. Each node decides which role (cluster-head or ordinary node) it wants to play based on the information it gathers from neighboring nodes. Before a node makes a decision about the role it plays, it waits for all neighboring nodes with a higher weight to make a decision. After a node decides about its role, it broadcasts the decision to all neighboring nodes. The node with the highest weight in every local community becomes the cluster-head of this community. All other nodes join the cluster-head with the highest weight as ordinary nodes. The time complexity of the \ac{DCA} depends on the network topology rather than on the size of the network. This approach leads to the following characteristics:
%\begin{itemize}
%	\item Every ordinary node has at least one neighboring cluster-head;
%	\item Every ordinary node joins the "best" neighboring cluster head;
%	\item There are no cluster-heads which are neighbors to each other.
%\end{itemize}
%
%Figure \ref{DCA_clustering_graph}a depicts a graph of a \ac{WSN}. Figure \ref{DCA_clustering_graph}b shows the clustered graph which is a result of the \ac{DCA}. In Figure \ref{DCA_clustering_graph} the unique node identifier is represented by its name, and the weights are denoted by (wn). As shown in Figure \ref{DCA_clustering_graph}b the node with the highest weight plays the role of the cluster-head in every cluster. It also shows that the three characteristics of the \ac{DCA} are satisfied.

\begin{figure}[t]
	\centering
	\includegraphics[scale=0.38]{pics/HCCA_clustering}      
	\caption{Cluster formation according to the \ac{HCC} algorithm. Each node ($v, u$) discovers its subtree size and forwards this information upstream to its parent. If the subtree size is big enough, the subtree becomes a cluster (A, B, C, D). (The Figure is redrawn from \cite{Banerjee2001})}
	\label{HCC_clustering_graph}
\end{figure}

The \ac{HCC} algorithm is a multi-tier hierarchical clustering algorithm which has proven to be highly scalable. The set-up phase involves the \ac{BFS} tree discovery and cluster formation. The tree discovery is a distributed formation of a \ac{BFS} tree rooted at the initiator node. The cluster formation is shown in Figure \ref{HCC_clustering_graph}. The clustering formation process is distributed and it is executed on each node. Based on the tree discovery each node knows its parent node and its child nodes. Each node $i$ discovers the size of its downstream subtree $|V_i|$ and reports this to its parent node. The information about the subtree sizes allows us to create the clusters based on the defined cluster size $k$ (number of nodes per cluster - this number is predefined). Each node compares its subtree size $|V_i|$ to the defined cluster size $k$ and if $k \leq |V_i| < 2k$ the node initiates the cluster formation on its subtree. As the \ac{BFS} tree denotes the routes to the base station, the sensing information of all sensors is transmitted using these routes. The maintenance phase involves just the maintaining up to date information on each node about its parent and child nodes. 
%After we define the cluster size (number of nodes in a cluster), the tree gets logically divided into clusters based on the size. 
%Figure \ref{HCA_clustering_graph} depicts the process of cluster creation according to the hierarchical control clustering algorithm. The process is distributed and it is executed on each node. First, the nodes discover the subtree size and forward this information upstream to its parent nodes. If the subtree size is big enough, the subtree becomes a cluster. If there is no node in the subtree of a node which is not assigned to a cluster, that node reports a subtree size of zero to its parent.
%The authors of \cite{Banerjee2001} propose a clustering scheme for hierarchical control in \ac{WSNs}. Hierarchical structures proved themselves as highly scalable, which makes them a good choice for \ac{WSNs}. In order to satisfy the requirements of \ac{WSNs} (e.g. connectivity, network longevity, fault-tolerance), the clustering algorithm should accomplish the following desired goals:
%\begin{itemize}
%	\item Each cluster is connected;
%	\item Each cluster should have a minimum and maximum size constraint;
%	\item A node in any layer of the hierarchy belongs to a constant number of clusters in that layer;
%	\item Two clusters should have low overlap;
%	\item Clusters should be stable across node mobility.
%\end{itemize}
%For more details about the listed goals the reader is referred to \cite{Banerjee2001}. Due to the size and ad-hoc connectivity of \ac{WSNs} a centralized approach does not seem justifiable. Hence, the authors of \cite{Banerjee2001} propose a distributed algorithm which allows them to perform the hierarchical clustering. We focus on the set-up phase of the algorithm. 
%The set-up phase consists of two parts: 
%\begin{itemize}
%	\item Tree Discovery - distributed implementation of the \ac{BFS} algorithm;
%	\item Cluster Formation - creates the clusters based on the \ac{BFS} tree.
%\end{itemize}
  


==> Clustering in WSNs Abstract/conclusion_section.tex <==
% !TeX spellcheck = en_US
Our analysis confirms the observation made by the authors of \cite{Jiang2009}, which highlights the trade-off between scalability and energy efficiency. With our complex systems science approach we showed that these aspects of different clustering algorithms can be analyzed together by analyzing the functional complexity of the specific implementation. Increasing values of $C_F$ lead to the increase of scalability and the decrease of energy efficiency. \textcolor{second}{Our ongoing work also confirms this trend, by analyzing other WSN clustering algorithms.}





==> Clustering in WSNs Abstract/functional_framework_section.tex <==
% !TeX spellcheck = en_US
\textcolor{activecolor}{We employ the functional framework introduced in \cite{Dzaferagic2016} to represent the implementation of the clustering algorithm with a functional topology. The functional topology is a graph that depicts the functional connectivity between system parts, where each node represents a functional entity related to the implementation, and each link indicates interactions between nodes.}

\textcolor{activecolor}{The functional complexity metric, also proposed in \cite{Dzaferagic2016}, is based on the Shannon entropy ($H(x_n)$) as a key characteristic of any system. To describe the potential for a node to interact with other nodes we employ the Bernoulli random variable $x_n$. The probability of interactions $p(x_n=1)$ is defined as the reachability of a node $n$ ($p_r(x_n=1) = i_r^n/j$, where $i_r^n$ is the number of nodes that can reach node $n$ and $j$ is the number of nodes for the given subgraph.}
%To quantify the variety of connection patterns between system entities and the roles that these entities have in the topology we employ a metric called functional complexity \cite{Dzaferagic2016}. 


%\begin{table}[t]
%	\centering
%	\caption{}
%	\label{tab:equation_notations}
%	\begin{tabular}{cp{\dimexpr 0.6\linewidth-2\tabcolsep}}
%		\toprule
%		\textbf{Symbol} & \textbf{Meaning}    \\[0.9ex]  \midrule
%		\centering{$n$} & node
%		\\[0.9ex]
%		\centering{$N$} & total number of nodes in the functional topology
%		\\[0.9ex] 
%		\centering{$j$} & subgraph size - number of nodes in the subgraph
%		\\[0.9ex] 
%		\centering{$r$} & scale size
%		\\[0.9ex] 
%		\centering{$R$} & maximum scale size, which is defined as the
%		longest shortest path in the whole functional topology
%		\\[0.9ex] 
%		\centering{$H(x_n)$} & entropy of node $n$ which indicates the
%		uncertainty of interactions of node $n$ in the operation of a
%		network function
%		\\[0.9ex] 
%		\centering{$\Lambda_k^j$} & $\mathrm{k^{th}}$ subgraph with $j$ nodes 
%		\\[0.9ex] 
%		\centering{$I_r(\Lambda^N)$} & the total amount of information of the subgraph with $N$ nodes for scale $r$
%		\\[0.9ex] 
%		\centering{$\langle  I_r(\Lambda^j) \rangle$} & the average amount of information over all subgraphs with the size $j$
%		\\[0.9ex] 
%		\bottomrule
%	\end{tabular}
%\end{table}

\textcolor{second}{Since we focus on one hop communication the complexity metric applied to our system turns out to be the following simplified single scale version of the general functional complexity expression introduced in \cite{Dzaferagic2016}, i.e.}
% Hence, we perform a single-scale analysis with a simplified version of equation (\ref{eq:complexity}), which is represented with equation (\ref{eq:single_scale_complexity}). 
%As \ac{WSNs} rely on the communication established between one hop neighbors, in our analysis the maximum scale size will be equal to $R = 2$.
\begin{equation}\label{eq:single_scale_complexity}
C_F = \displaystyle\sum_{j = 2}^{N} | \langle I(\Lambda^j) \rangle - \dfrac{j}{N}  I(\Lambda^N)|,
\end{equation}
\textcolor{activecolor}{where $N$ is the total number of nodes in the functional topology and $\Lambda^j$ is a subgraph with $j$ nodes. The functional complexity compares the average uncertainty of interactions for a smaller subset ($\langle I(\Lambda^j) \rangle$) to the amount of information which is expected from the calculation performed on the whole system ($I(\Lambda^N)$).}

\textcolor{second}{$I(\Lambda^N)$ is the total amount of information of the whole functional topology. $I(\Lambda_k^j)$ is the uncertainty of interactions for a smaller subset, i.e. the total amount of information of the  $\mathrm{k^{th}}$ subgraph with $j$ nodes. It is calculated with equation (\ref{eq:total_amount_of_information}).}

\begin{equation}\label{eq:total_amount_of_information}
I(\Lambda_k^j) = \displaystyle\sum_{n \in \Lambda_k^j} H(x_n)
\end{equation}

$H(x_n)$ reaches its maximum if the probability of interaction with node $n$ is $p(x_n = 1) = 1/2$. As the distribution of links among nodes for a sparse graph is almost uniform, a sparse graph results in high values of $H(x_n)$. High values of $H(x_n)$ result in high values of $I(\Lambda_k^j)$. Therefore, the functional complexity is high for a sparse graph, with uniformly distributed links among nodes for subgraphs with the size $j < N$. The functional complexity is zero for a fully connected and for a disconnected graph. For more details about the functional framework and the complexity metric expressed by equation (\ref{eq:single_scale_complexity}) the reader is referred to \cite{Dzaferagic2016}. 
%Therefore, the functional complexity is high for a sparse graph with a uniform distribution of links. The functional complexity also depends on the distribution of links for smaller subgraphs. If the distribution of links among nodes for smaller subgraphs is close to a uniform distribution, the uncertainty of interactions for these subgraphs becomes much higher than it would be expected from the uncertainty of the whole graph. 

\textcolor{activecolor}{The physical topology of our \ac{WSN} is created according to the Von Neumann neighborhood, which is basically an undirected lattice graph. Now we employ our functional framework to represent the implementation of the \ac{HCC} algorithm as a functional topology. Our goal is to investigate the influence of the interactions among nodes after the clusters are established, on the objectives of clustering algorithms (\textcolor{second}{i.e. scalability and energy efficiency}). We focus on the maintenance phase of the algorithm. After the set-up phase the nodes establish connections to their neighboring nodes according to the \ac{BFS} algorithm. Each node discovers its subtree, and exchanges information with its neighbors in the \ac{BFS} tree. We imagine a virtual decision maker entity that is moving from one node to another. At each node the decision maker entity collects information from nodes that belong to its subtree  and forwards this information to its parent. In other words, each node maintains its position in the \ac{BFS} tree and therefore the functional topology of the \ac{HCC} algorithm is equivalent to the \ac{BFS} tree created upon the physical topology (Figure \ref{functional_topology_HCCA}).}


\begin{figure}[t]
	\centering
	\includegraphics[scale=0.4]{pics/functional_topology_HCCA}      
	\caption{The functional topology of the \ac{HCC} algorithm for a network of twenty nodes, which represents the \ac{BFS} tree created based on the physical topology. The white nodes represent ordinary nodes, the black nodes represent cluster-heads, and the gray node represents the base station. }
	\label{functional_topology_HCCA}
\end{figure}





%TODO
%DONE - emhasize that we use a modified equation to calculate complexity, which means that we calculate single scale complexity (for the scale r=2)
%DONE - introduce the functional topology framework - reference our paper
%DONE - say something about the complex systems science approach 
%DONE - mention the complexity metric that we are going to use
%DONE - cite the functional framework paper (our paper)
%DONE - define the graph that is going to be used  - physical topology
%DONE - add figure of the physical topology
%DONE - describe the process of creating functional topologies for the two chosen algorithms - use the virtual decision maker entity 
%DONE - add figures of the functional topologies


==> Clustering in WSNs Abstract/introduction_section.tex <==
% !TeX spellcheck = en_US
%In addition to the energy efficiency, which explicitly affects the network lifetime, clustering algorithms have a great influence on scalability, load balancing, fault-tolerance, delay reduction, etc. \cite{Abbasi2007}. 
%TODO chose the literature ---- max 10 papers better less
Clustering partitions a network of nodes into a number of smaller groups (clusters). Different approaches to clustering are available in the literature. The authors of \cite{Abbasi2007, Liu2012, Aslam2012, Banerjee2001} introduced different approaches, which involve adaptive clustering, random competition based clustering, \ac{HCC}, energy efficient hierarchical clustering, distributed clustering, \ac{LEACH}, and \ac{HEED} clustering. They also highlighted that the algorithms differ in properties like stability of the created clusters, objectives (e.g. scalability, fault-tolerance, connectivity, load balancing, redundancy elimination, rapid convergence, network lifetime), clustering criteria (e.g. identifier, position, cluster head frequency, residual energy), methodology (e.g. distributed, centralized, hybrid). \textcolor{activecolor}{Even though these algorithms are well studied, the analysis is missing an important aspect which involves the understanding of the mechanisms that lead to certain properties of these algorithms. Since the \ac{HCC} algorithm proposed in \cite{Banerjee2001} is the most popular multi-tier hierarchical clustering algorithm \cite{Abbasi2007}, in the course of this analysis we will focus on this algorithm.}

Understanding the organizational and communication characteristics of different clustering algorithms allows us to comprehend which aspects of a specific implementation lead to certain characteristics, i.e. scalability and energy efficiency. In \cite{Dzaferagic2016}, we propose a framework which allows us to represent network functions with graphs called functional topologies. Therein, we also propose a metric to calculate the functional complexity of an implementation of a network function. Here, we employ our functional framework to model an implementation for clustering in \ac{WSNs}. \textcolor{second}{Our goal is to investigate the relationship between the functional complexity and certain properties of the implementation, such as scalability and energy efficiency}. This allows us to understand the underlying mechanisms that are a product of complex interactions between functional entities.
%Our goal is to highlight the structural patterns present in the functional topology that result in certain properties of the implementation. 

%TODO use this to explain the equation
%The complex systems science approach we adopt allows us to investigate the amount of information about the system subparts by examining the system as a whole and comparing this to the actual amount of information that exists within the system subparts. In other words, this allows us to quantify the amount of uncertainty of interaction that exists within smaller subparts of the system compared to the uncertainty of the whole system.
%TODO use this for the conclusion
%The main contributions of this paper are:
%\begin{itemize}
%	\item We apply a complex systems science approach to analyze clustering in \ac{WSNs};
%	\item Our study shows how the density of local connections in the functional topology affects the scalability of a clustering implementation;
%	\item Our results highlight the structural patterns in the functional topology that lead to higher energy efficiency of the WSN;
%	\item Our functional complexity allows us to analyze the trade-off between energy efficiency and scalability of a clustering implementation.
%\end{itemize}


==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Communications Society subset of the full
IEEEtran package and is intended for use with IEEE Communications Society
publications. The included version of the IEEEtran_HOWTO.pdf has been
specially formatted in IEEE Communications Society (comsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf,
                   bare_jrnl_comsoc.tex.
***************************************************************************


==> clustering_algorithms_section.tex <==
% !TeX spellcheck = en_US
%The importance of collecting, analyzing and interpreting data in the \ac{IoT} environment emphasizes the role of \ac{WSNs}. A WSN is a collection of connected devices (sensors), which can sense the environment, interpret the measurements and communicate this information through the network. In order to make the measurements as precise as possible, and the network as reliable as possible, \ac{WSNs} generally possess a large number of sensors. Therefore, in addition to the sensing and communication abilities, sensors have to be cheap. In order to make these devices as cheap as possible, their capabilities are limited (e.g. sensors have limited energy resources, which explicitly influences every aspect of \ac{WSNs}). 

Considering the limited energy resources and the size of \ac{WSNs}, the best approach is to partition the network into interconnected subgroups (clusters), whose local behavior gives rise to the global objective of the network (e.g. minimizing the energy consumption). Generally, clustering includes two phases:
\begin{itemize}
	\item Set-Up Phase - this phase implies choosing cluster-heads. Cluster-heads are nodes that are responsible for the coordination of the clustering process.
	\item Maintenance Phase - this phase implies reorganization of the clusters in order to add new nodes to the cluster, deal with nodes that leave the cluster, or simply change the roles of nodes (cluster-head or ordinary node) in the cluster in order to achieve higher energy efficiency \cite{Basagni1999}. 
\end{itemize}

%We propose a complex systems science approach to understand how different clustering approaches lead to specific network properties (in particular we focus on scalability and energy efficiency). 
As the maintenance phase implies the reorganization of clusters in order to achieve higher energy efficiency and to adjust to changes in the topology, we focus on this phase. As mentioned previously, we consider two clustering algorithms (the \ac{LEACH} and the \ac{HCC} algorithms) proposed in \cite{Heinzelman2002} and \cite{Banerjee2001}.

\begin{figure}[t]
	\centering
	\includegraphics[scale=0.4]{pics/leach_clustering}      
	\caption{The topology created according to the \ac{LEACH} algorithm. Ordinary nodes transfer sensing information to the cluster-heads, which forward this information to the base station (The Figure is redrawn from \cite{Aslam2012})}
	\label{leach_clustering_graph}
\end{figure}

The \ac{LEACH} algorithm is based on rounds. Each round includes both phases (set-up and maintenance phase). Each node in the network runs the algorithm, and decides randomly which role to play (cluster-head or ordinary node). When a node decides to be a cluster-head it broadcasts this information, whereas each node that decided to be an ordinary node listens to the broadcast messages and joins the closest cluster-head. After all ordinary nodes join one of the cluster-heads, the set-up phase finishes and the maintenance phase starts. In the maintenance phase nodes that belong to the same cluster transfer sensing information to the cluster-head (Figure \ref{leach_clustering_graph}), and as the \ac{LEACH} algorithm involves rotating the role of cluster-heads between nodes in a cluster, the nodes that belong to the same cluster communicate to each other in order to choose the next cluster-head candidate. 
%The \ac{DCA} generalizes algorithms presented in \cite{Lin1997} and \cite{Baker1981}, by choosing the cluster-heads based on a generic weight associated with each node. Each node executes the algorithm, and each node has the knowledge of its unique identifier, its weight, and the weights and unique identifiers of its neighboring nodes. In other words, the algorithm relies only on local information. Each node decides which role (cluster-head or ordinary node) it wants to play based on the information it gathers from neighboring nodes. Before a node makes a decision about the role it plays, it waits for all neighboring nodes with a higher weight to make a decision. After a node decides about its role, it broadcasts the decision to all neighboring nodes. The node with the highest weight in every local community becomes the cluster-head of this community. All other nodes join the cluster-head with the highest weight as ordinary nodes. The time complexity of the \ac{DCA} depends on the network topology rather than on the size of the network. This approach leads to the following characteristics:
%\begin{itemize}
%	\item Every ordinary node has at least one neighboring cluster-head;
%	\item Every ordinary node joins the "best" neighboring cluster head;
%	\item There are no cluster-heads which are neighbors to each other.
%\end{itemize}
%
%Figure \ref{DCA_clustering_graph}a depicts a graph of a \ac{WSN}. Figure \ref{DCA_clustering_graph}b shows the clustered graph which is a result of the \ac{DCA}. In Figure \ref{DCA_clustering_graph} the unique node identifier is represented by its name, and the weights are denoted by (wn). As shown in Figure \ref{DCA_clustering_graph}b the node with the highest weight plays the role of the cluster-head in every cluster. It also shows that the three characteristics of the \ac{DCA} are satisfied.

\begin{figure}[t]
	\centering
	\includegraphics[scale=0.38]{pics/HCCA_clustering}      
	\caption{Cluster formation according to the \ac{HCC} algorithm. Each node ($v, u$) discovers its subtree size and forwards this information upstream to its parent. If the subtree size is big enough, the subtree becomes a cluster (A, B, C, D). (The Figure is redrawn from \cite{Banerjee2001})}
	\label{HCC_clustering_graph}
\end{figure}

The \ac{HCC} algorithm is a multi-tier hierarchical clustering algorithm which has proven to be highly scalable. The set-up phase involves the \ac{BFS} tree discovery and cluster formation. The tree discovery is a distributed formation of a \ac{BFS} tree rooted at the initiator node. The cluster formation is shown in Figure \ref{HCC_clustering_graph}. The clustering formation process is distributed and it is executed on each node. Based on the tree discovery each node knows its parent node and its child nodes. Each node $i$ discovers the size of its downstream subtree $|V_i|$ and reports this to its parent node. The information about the subtree sizes allows us to create the clusters based on the defined cluster size $k$ (number of nodes per cluster - this number is predefined). Each node compares its subtree size $|V_i|$ to the defined cluster size $k$ and if $k \leq |V_i| < 2k$ the node initiates the cluster formation on its subtree. As the \ac{BFS} tree denotes the routes to the base station, the sensing information of all sensors is transmitted using these routes. The maintenance phase involves just the maintaining up to date information on each node about its parent and child nodes. 
%After we define the cluster size (number of nodes in a cluster), the tree gets logically divided into clusters based on the size. 
%Figure \ref{HCA_clustering_graph} depicts the process of cluster creation according to the hierarchical control clustering algorithm. The process is distributed and it is executed on each node. First, the nodes discover the subtree size and forward this information upstream to its parent nodes. If the subtree size is big enough, the subtree becomes a cluster. If there is no node in the subtree of a node which is not assigned to a cluster, that node reports a subtree size of zero to its parent.
%The authors of \cite{Banerjee2001} propose a clustering scheme for hierarchical control in \ac{WSNs}. Hierarchical structures proved themselves as highly scalable, which makes them a good choice for \ac{WSNs}. In order to satisfy the requirements of \ac{WSNs} (e.g. connectivity, network longevity, fault-tolerance), the clustering algorithm should accomplish the following desired goals:
%\begin{itemize}
%	\item Each cluster is connected;
%	\item Each cluster should have a minimum and maximum size constraint;
%	\item A node in any layer of the hierarchy belongs to a constant number of clusters in that layer;
%	\item Two clusters should have low overlap;
%	\item Clusters should be stable across node mobility.
%\end{itemize}
%For more details about the listed goals the reader is referred to \cite{Banerjee2001}. Due to the size and ad-hoc connectivity of \ac{WSNs} a centralized approach does not seem justifiable. Hence, the authors of \cite{Banerjee2001} propose a distributed algorithm which allows them to perform the hierarchical clustering. We focus on the set-up phase of the algorithm. 
%The set-up phase consists of two parts: 
%\begin{itemize}
%	\item Tree Discovery - distributed implementation of the \ac{BFS} algorithm;
%	\item Cluster Formation - creates the clusters based on the \ac{BFS} tree.
%\end{itemize}
  

